Learning with Noisy Labels by Adaptive Gradient-Based Outlier Removal

An accurate and substantial dataset is essential for training a reliable and well-performing model. However, even manually annotated datasets contain label errors, not to mention automatically labeled ones. Previous methods for label denoising have primarily focused on detecting outliers and their permanent removal - a process that is likely to over- or underfilter the dataset. In this work, we propose AGRA: a new method for learning with noisy labels by using Adaptive GRAdient-based outlier removal. Instead of cleaning the dataset prior to model training, the dataset is dynamically adjusted during the training process. By comparing the aggregated gradient of a batch of samples and an individual example gradient, our method dynamically decides whether a corresponding example is helpful for the model at this point or is counter-productive and should be left out for the current update. Extensive evaluation on several datasets demonstrates AGRA's effectiveness, while a comprehensive results analysis supports our initial hypothesis: permanent hard outlier removal is not always what model benefits the most from.

==> algorithms/02_multi_label.tex <==
\begin{algorithm}[H]
\textbf{Input:} training set $\mathcal{X}$, initial model $f(\cdot; \theta)$, number of epochs $E$, batch size $M$, number of classes $K$, label assigned to ignored samples $i$ \\
\textbf{Output:} trained model $f(\cdot; \theta^*)$ \\
%\textbf{Output}: trained model $f(\cdot; \theta^*)$ \\
\For{epoch = 1,..., $E$}{
 \For{batch $\mathcal{B}$}{
  Sample a comparison batch $\widetilde{\mathcal{B}}$, $\widetilde{\mathcal{B}} \subset \mathcal{X}$, $|\widetilde{\mathcal{B}}| = M$\\
  Compute $\nabla\widetilde\mathcal{L}_{c}$ on $\widetilde{\mathcal{B}}$\\
  \For{($x_t$, $y_t$) $\in$ $\mathcal{B}$}{
  Compute $\nabla\widetilde\mathcal{L}_{(x_t,y_t)}$ wrt. $\widetilde{\mathcal{L}}$ \\
  Set up corrected label vector $y_t^* \leftarrow y_t$ \\
  \For{k=1, ..., $K$}{
    $sim_{y_t}^k = sim((\nabla\widetilde\mathcal{L}_{(x_t,y_t)})_{k}, (\nabla\widetilde\mathcal{L}_{c})_{k})$ (Eq.\ref{sim}) \\
    \If {$sim_{y_t}^k \leq \tau$}{
        $y^*_{t,k} \leftarrow i$}}
        $\mathcal{B} \leftarrow \left(\mathcal{B} \setminus \{(x_t, y_t)\}\right) \cup \{(x_t, y_t^*)\}$
    
  }
  %Update $\theta$ wrt. $\mathcal{L}$ and $\mathcal{B}$\;
  $\theta \leftarrow Optimizer(\theta, \mathcal{B}, \mathcal{L})$
 }
 }
\caption{GM Algorithm for Multi-Label Datasets}
\label{alg:alg_multi}
\end{algorithm}

==> tables/02_dataset_stat.tex <==
\begin{table}[H]
\centering
\begin{tabular}{lrrrrrr}
\hline
 Dataset &  \#Class &   \#Train & \#Dev &  \#Test & \%Noise \\
\hline
 YouTube &          2 &      1586 &    120 &     250 &     18.8\\
     SMS &          2 &      4571 &    500 &     500 &      31.9\\
    TREC &          6 &      4965 &    500 &     500 &      48.2\\
Yorùb\'a &          7 &      1340 &    189 &     379 &      42.3\\
   Hausa &          5 &      2045 &    290 &     582 &      50.6\\
CheXpert &         12 &    200599 &  22815 &     234 &      -\\
\hline
\end{tabular}
\caption{Datasets statistics. 
Percentage of noise is calculated by comparing the noisy labels to the gold-standard annotations.  
%Coverage is computed on the train set by dividing the number of samples having at least one match by the number of samples. 
}
\label{table:dataset_stats}
\end{table}

==> tables/02_results_tfidf_img.tex <==
\begin{table}
\centering
\begin{tabular}{lcc|c}
& \multicolumn{1}{p{2cm}}{\centering \textbf{CIFAR-10} \\ \small{(Acc)}}
& \multicolumn{1}{p{2cm}|}{\centering \textbf{CheXpert} \\ \small{(AUROC)}}
& {\centering \textbf{Avg.}}
\\
\hline
\hline %\xrowht[()]{5pt}
%\textit{Gold data}   & & & & & & & \\%\xrowht[()]{5pt}
Gold & & - & \\
% \hline%\xrowht[()]{5pt}
% \textit{Noisy data}              & & & & & & & \\%\xrowht[()]{5pt}
% MV - with GM baseline script   & $95.1 \pm 0.5$ & $76.1 \pm 2.0$ & $60.5 \pm 0.5$ & $49.2 \pm 1.3$ & $43.1 \pm 0.3$ &\\
No Denoising & & $82.7 \pm 0.1$ & \\%\xrowht[()]{5pt}
\hline
\textit{Noisy Learning} &&& \\
% MentorNet &&& \\
CORES$^2$ && - & \\
Cleanlab \small{\cite{northcutt2021confident}} && $81.1 \pm 0.2$ &\\
\hline%\xrowht[()]{5pt}
\textbf{\name} & & $\textbf{83.9} \pm 0.3$ & \\%\xrowht[()]{5pt}
\end{tabular}
% \captionsetup{justification=centering}
\caption{Experimental results on image datasets averaged across five runs and reported with standard deviation.
%Results marked with $^*$ are statistically significant (more details on significance testing are provided in Appendix F).
}
\label{tab:results}
\end{table}



%%%%% new Yoruba results (F1 macro metric)
% Gold: 57.3 \pm 0.4
% MV: 44.6 \pm 0.4
% FS: 31.9 \pm 0.7
% DP: 47.8 \pm 1.7
% Cleanlab: 32.9 \pm 1.5
% GM: 48.2 \pm 2.7; 
% GM params: lr = 0.1, batch_size = 512, decay = 1e-05, threh = 0, weights=False, train_loss = CE, comp_loss = F1 


%%%%% new Hausa results (F1 macro metric)
% Gold: 78.5 \pm 03
% MV: 39.7 \pm 0.8
% FS: 37.6 \pm 1.0
% DP: 40.9 \pm 0.6
% Cleanlab: 37.1 \pm 0.5
% GM: 
% GM params: 






% \textit{Manually labeled data}   & & & & & & & \\%\xrowht[()]{5pt}
% Gold                             & $94.8 \pm 0.8$ & $95.4 \pm 1.0$ & $89.5 \pm 0.3$ & $68.5 \pm 1.3$ & $78.5 \pm 0.3$ & $85.3$ & - \\
% \hline%\xrowht[()]{5pt}
% \textit{Noisy data}              & & & & & & & \\%\xrowht[()]{5pt}
% MV - with GM baseline script   & $95.1 \pm 0.5$ & $76.1 \pm 2.0$ & $60.5 \pm 0.5$ & $49.2 \pm 1.3$ & $43.1 \pm 0.3$ &\\
% MV                               & $87.4 \pm 2.7$ & $71.7 \pm 1.4$ & $58.7 \pm 0.5$ & $47.9 \pm 0.4$ & $43.3 \pm 0.3$ & $61.8$ & \\%\xrowht[()]{5pt}
% FlyingSquid \small{\cite{pmlr-v119-fu20a}} & $84.8 \pm 1.5$ & $16.3 \pm 6.0$ & $27.2 \pm 0.1$ & $\textbf{59.6} \pm 0.4$ & $41.7 \pm 0.8$ & $57.6$ & - \\%\xrowht[()]{5pt}
% DP \small{\cite{ratner2016data}} & $90.8 \pm 1.0$ & $44.1 \pm 6.7$ & $54.3 \pm 0.5$ & $58.2 \pm 0.5$ & $42.9 \pm 0.6$ & $58.1$ & - \\%\xrowht[()]{5pt}
%Cleanlab \small{(Northcutt et al. 2021)} & $89.6 \pm 0.6$ & $63.7 \pm 1.5$ & $58.5 \pm 0.3$ & $39.3 \pm 0.7$ & $41.8 \pm 0.3$ & $58.6$ & \\
% \hline%\xrowht[()]{5pt}
% \textbf{\name} & $\textbf{95.4} \pm 0.4$ & $\textbf{84.8} \pm 1.1$ & $\textbf{63.5} \pm 0.6$ & $55.6 \pm 2.2$ & $\textbf{52.0} \pm 0.7$ & $\textbf{70.2}$ & \\%\xrowht[()]{5pt}
% \captionsetup{justification=centering}


==> tables/03_large_table_aaai.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{l|c|c|c|c|c|c}%\xrowht[()]{10pt}
&
\multicolumn{3}{c}{No Weighted Sampling}&
\multicolumn{3}{|c}{Weighted Sampling}
\\
\hline
\hline\xrowht[()]{5pt} &
\multicolumn{1}{p{1.5cm}|}{\centering CE/CE}&
\multicolumn{1}{p{1.5cm}|}{\centering CE/$F_{1}$}&
\multicolumn{1}{p{1.5cm}|}{\centering $F_{1}$/CE}&
% \multicolumn{1}{p{1.5cm}|}{\centering $F_{1}$/$F_{1}$}&
\multicolumn{1}{p{1.5cm}|}{\centering CE/CE}&
\multicolumn{1}{p{1.5cm}|}{\centering CE/$F_{1}$}&
\multicolumn{1}{p{1.5cm}}{\centering $F_{1}$/CE}
% \multicolumn{1}{p{1.5cm}}{\centering $F_{1}$/$F_{1}$}  \xrowht[()]{8pt}
\\
\hline
YouTube & 
$94.2 \pm 0.2$ & 
$92.0 \pm 0.8$ & 
$94.6 \pm 0.8$ &
%$94.8 \pm 0.6$ & 
$94.0 \pm 0.0$ & 
$92.9 \pm 0.4$ &
$\textbf{95.0} \pm 0.5$
% $\textbf{95.4} \pm 0.5$ 
\\ %\xrowht[()]{5pt}
YouTube^\dagger & 
$93.0 \pm 2.0$ &
$93.9 \pm 1.1$ & 
$78.8 \pm 8.6$ & 
% $94.0 \pm 1.0$ & 
$89.2 \pm 4.3$ &
$92.3 \pm 0.9$ & 
$78.3 \pm 7.6$ 
% $92.4 \pm 0.7$ 
\\%\xrowht[()]{5pt}
SMS & 
$77.9 \pm 1.8$ & 
$\textbf{84.8 \pm 1.1}$ & 
$52.7 \pm 2.0$ & 
%$48.1 \pm 1.4$ & 
$80.9 \pm 0.7$ & 
$84.6 \pm 1.0$ &
$47.0 \pm 1.2$
%$48.0 \pm 1.0$ 
\\%\xrowht[()]{5pt}
SMS^\dagger & 
$70.8 \pm 2.7$ & 
$74.5 \pm 1.6$ & 
$28.1 \pm 5.7$ & 
%$39.7 \pm 0.6$ & 
$78.9 \pm 1.9$ & 
$74.0 \pm 2.0$ & 
$28.3 \pm 2.0$
%$41.1 \pm 0.5$ 
\\ %\xrowht[()]{5pt}
TREC & 
$61.2 \pm 0.8$ & 
$61.4 \pm 0.3$ &
$60.3 \pm 1.1$ &
% $60.8 \pm 0.6$ & 
$63.2 \pm 0.5$ &
$62.8 \pm 0.6$ & 
$\textbf{63.5} \pm 0.6$ 
% $62.3 \pm 0.5$ 
\\%\xrowht[()]{5pt}
Yorùb\'a & 
$43.5 \pm 0.6$ & 
$\textbf{48.2 }\pm 2.7$ & 
$44.8 \pm 1.2$ & 
%$44.3 \pm 2.6$ & 
$45.2 \pm 0.8$ & 
$44.7 \pm 0.4$ & 
$44.4 \pm 1.5$ 
%$45.5 \pm 1.3$ 
\\%\xrowht[()]{5pt}
Hausa & 
$40.6 \pm 0.3$ & 
$39.7 \pm 2.0$ & 
$41.7 \pm 1.2$ & 
% $41.0 \pm 0.8$ & 
$46.3 \pm 2.7$ & 
$\textbf{50.9 }\pm 1.1$ & 
$49.3 \pm 1.4$
% $48.7 \pm 1.2$ 
\\%\xrowht[()]{5pt}
CheXpert & 
$ 82.2 \pm 0.1$ & 
$83.2 \pm 0.1$ & 
$83.7 \pm 0.1$ & 
% $\textbf{83.9} \pm 0.3$ & 
$-$ & 
$-$ & 
$-$
% $-$ 
\\%\xrowht[()]{5pt}
\end{tabular}
% \captionsetup{justification=centering}
\caption{\name experimental results with different settings: use of class-weighted sampling, [training loss]/[comparison loss]. 
The results marked with $\dagger$ are obtained by \name with an alternative label.
% Binary cross-entropy was used for the experiments on CheXpert dataset.
All results are averaged across 5 runs and reported with standard deviation.}
\label{tab:all_results}
\end{table}



% SMS F1/F1+no_weighting: 48.0 ± 0.2 -> 48.1 ± 1.4
% SMS F1/F1+weighting: 47.9 ± 0.2 -> 48.0 ± 1.0
% Yoruba CE/CE+no weighting: 51.3 ± 4.5 -> ±
% Yoruba F1/F1+no weighting: 51.5 ± 4.4 -> 53.2 ± 3.5
% Yoruba F1/F1+ weighting: 52.6 ± 0.9  -> ±

%Just ran yoruba for the plots, with some seeds almost 10% accuracy less (46) 




% YouTube & $91.8 \pm 0.7$ & $92.0 \pm 0.8$ & $94.6 \pm 0.8$ & $94.8 \pm 0.6$ & $91.7 \pm 0.5$ & $92.9 \pm 0.4$& $95.0 \pm 0.5$& $95.4 \pm 0.5$\\%\xrowht[()]{5pt}
% SMS & $74.5 \pm 1.7$ & $84.8 \pm 1.1$ & $52.7 \pm 2.0 $& $48.1 \pm 1.4$ & $80.9 \pm 0.7$ & $84.6 \pm 1.0 $& $47.0 \pm 1.2 $&$ 48.0 \pm 1.0$\\%\xrowht[()]{5pt}
% TREC & $61.6 \pm 0.8$ & $61.4 \pm 0.3$ & $60.3 \pm 1.1$ & $60.8 \pm 0.6$ & $63.2 \pm 0.5$ &$62.8 \pm 0.6 $& $63.5 \pm 0.6$ & $62.3 \pm 0.5$\\%\xrowht[()]{5pt}
% Yorùb\'a & $51.3 \pm 4.5 ?$ & $55.6\pm 2.2$ & $48.2 \pm 1.7$ & $53.2 \pm 3.5$& $49.8 \pm 0.8 $& $51.4 \pm 1.5 $& $51.5 \pm 2.5$ & $52.6 \pm 0.9 ?$\\%\xrowht[()]{5pt}
% Hausa & $44.2 \pm 0.6$ & $44.3 \pm 0.5 $& $42.8 \pm 0.0 $&$ 43.8 \pm 0.5 $& $46.5 \pm 1.5 $&$ 49.4 \pm 1.7 $& $50.4 \pm 0.7$ & $52.0 \pm 0.7$\\

